Measurement of the Spin-Orbit Angle of Exoplanet HAT-P-1b

We present new spectroscopic and photometric observations of the HAT-P-1 planetary system. Spectra obtained during three transits exhibit the Rossiter-McLaughlin effect, allowing us to measure the angle between the sky projections of the stellar spin axis and orbit normal, \lambda = 3.7 +/- 2.1 degrees. The small value of \lambda for this and other systems suggests that the dominant planet migration mechanism preserves spin-orbit alignment. Using two new transit light curves, we refine the transit ephemeris and reduce the uncertainty in the orbital period by an order of magnitude. We find a upper limit on the orbital eccentricity of 0.067, with 99% confidence, by combining our new radial-velocity measurements with those obtained previously.

==> table_phot.tex <==
  $  1$  &  $  2454381.71537$  &  $  0.9988$ \\
  $  1$  &  $  2454381.71588$  &  $  1.0002$ \\
  $  1$  &  $  2454381.71640$  &  $  1.0007$ \\
  $  1$  &  $  2454381.71691$  &  $  1.0028$ \\
  $  1$  &  $  2454381.71904$  &  $  1.0018$ \\
  $  1$  &  $  2454381.71955$  &  $  1.0002$ \\
  $  1$  &  $  2454381.72007$  &  $  1.0031$ \\
  $  1$  &  $  2454381.72058$  &  $  1.0009$ \\
  $  1$  &  $  2454381.72110$  &  $  0.9989$ \\
  $  1$  &  $  2454381.72161$  &  $  0.9991$ \\
  $  1$  &  $  2454381.72213$  &  $  1.0001$ \\
  $  1$  &  $  2454381.72264$  &  $  0.9982$ \\
  $  1$  &  $  2454381.72316$  &  $  0.9985$ \\
  $  1$  &  $  2454381.72367$  &  $  0.9998$ \\
  $  1$  &  $  2454381.72419$  &  $  0.9998$ \\
  $  1$  &  $  2454381.72470$  &  $  0.9990$ \\
  $  1$  &  $  2454381.72522$  &  $  1.0004$ \\
  $  1$  &  $  2454381.72573$  &  $  1.0021$ \\
  $  1$  &  $  2454381.72625$  &  $  1.0002$ \\
  $  1$  &  $  2454381.72676$  &  $  1.0015$ \\
  $  1$  &  $  2454381.72728$  &  $  1.0038$ \\
  $  1$  &  $  2454381.72780$  &  $  1.0038$ \\
  $  1$  &  $  2454381.72831$  &  $  0.9986$ \\
  $  1$  &  $  2454381.72883$  &  $  1.0020$ \\
  $  1$  &  $  2454381.73073$  &  $  0.9991$ \\
  $  1$  &  $  2454381.73125$  &  $  1.0050$ \\
  $  1$  &  $  2454381.73176$  &  $  1.0005$ \\
  $  1$  &  $  2454381.73228$  &  $  1.0002$ \\
  $  1$  &  $  2454381.73279$  &  $  1.0002$ \\
  $  1$  &  $  2454381.73331$  &  $  1.0023$ \\
  $  1$  &  $  2454381.73382$  &  $  1.0023$ \\
  $  1$  &  $  2454381.73434$  &  $  0.9986$ \\
  $  1$  &  $  2454381.73485$  &  $  1.0015$ \\
  $  1$  &  $  2454381.77500$  &  $  0.9890$ \\
  $  1$  &  $  2454381.77559$  &  $  0.9900$ \\
  $  1$  &  $  2454381.77609$  &  $  0.9860$ \\
  $  1$  &  $  2454381.77658$  &  $  0.9917$ \\
  $  1$  &  $  2454381.77707$  &  $  0.9881$ \\
  $  1$  &  $  2454381.77756$  &  $  0.9878$ \\
  $  1$  &  $  2454381.77805$  &  $  0.9882$ \\
  $  1$  &  $  2454381.77855$  &  $  0.9869$ \\
  $  1$  &  $  2454381.77904$  &  $  0.9878$ \\
  $  1$  &  $  2454381.77953$  &  $  0.9899$ \\
  $  1$  &  $  2454381.78002$  &  $  0.9886$ \\
  $  1$  &  $  2454381.78104$  &  $  0.9873$ \\
  $  1$  &  $  2454381.78154$  &  $  0.9862$ \\
  $  1$  &  $  2454381.78205$  &  $  0.9886$ \\
  $  1$  &  $  2454381.78255$  &  $  0.9905$ \\
  $  1$  &  $  2454381.78305$  &  $  0.9869$ \\
  $  1$  &  $  2454381.78356$  &  $  0.9859$ \\
  $  1$  &  $  2454381.78406$  &  $  0.9864$ \\
  $  1$  &  $  2454381.78456$  &  $  0.9874$ \\
  $  1$  &  $  2454381.78506$  &  $  0.9864$ \\
  $  1$  &  $  2454381.78557$  &  $  0.9864$ \\
  $  1$  &  $  2454381.78632$  &  $  0.9842$ \\
  $  1$  &  $  2454381.78682$  &  $  0.9858$ \\
  $  1$  &  $  2454381.78732$  &  $  0.9883$ \\
  $  1$  &  $  2454381.78783$  &  $  0.9864$ \\
  $  1$  &  $  2454381.78833$  &  $  0.9899$ \\
  $  1$  &  $  2454381.78883$  &  $  0.9879$ \\
  $  1$  &  $  2454381.78934$  &  $  0.9876$ \\
  $  1$  &  $  2454381.78984$  &  $  0.9860$ \\
  $  1$  &  $  2454381.79034$  &  $  0.9856$ \\
  $  1$  &  $  2454381.79085$  &  $  0.9833$ \\
  $  1$  &  $  2454381.79135$  &  $  0.9872$ \\
  $  1$  &  $  2454381.79185$  &  $  0.9849$ \\
  $  1$  &  $  2454381.79236$  &  $  0.9856$ \\
  $  1$  &  $  2454381.79286$  &  $  0.9869$ \\
  $  1$  &  $  2454381.79336$  &  $  0.9868$ \\
  $  1$  &  $  2454381.79387$  &  $  0.9875$ \\
  $  1$  &  $  2454381.79437$  &  $  0.9880$ \\
  $  1$  &  $  2454381.79487$  &  $  0.9880$ \\
  $  1$  &  $  2454381.79538$  &  $  0.9849$ \\
  $  1$  &  $  2454381.79588$  &  $  0.9852$ \\
  $  1$  &  $  2454381.79657$  &  $  0.9859$ \\
  $  1$  &  $  2454381.79707$  &  $  0.9846$ \\
  $  1$  &  $  2454381.79758$  &  $  0.9858$ \\
  $  1$  &  $  2454381.79808$  &  $  0.9869$ \\
  $  1$  &  $  2454381.79858$  &  $  0.9860$ \\
  $  1$  &  $  2454381.79909$  &  $  0.9861$ \\
  $  1$  &  $  2454381.79959$  &  $  0.9874$ \\
  $  1$  &  $  2454381.80009$  &  $  0.9861$ \\
  $  1$  &  $  2454381.80060$  &  $  0.9843$ \\
  $  1$  &  $  2454381.80110$  &  $  0.9849$ \\
  $  1$  &  $  2454381.80180$  &  $  0.9872$ \\
  $  1$  &  $  2454381.80230$  &  $  0.9881$ \\
  $  1$  &  $  2454381.80280$  &  $  0.9874$ \\
  $  1$  &  $  2454381.80331$  &  $  0.9848$ \\
  $  1$  &  $  2454381.80381$  &  $  0.9861$ \\
  $  1$  &  $  2454381.80431$  &  $  0.9834$ \\
  $  1$  &  $  2454381.80482$  &  $  0.9851$ \\
  $  1$  &  $  2454381.80532$  &  $  0.9863$ \\
  $  1$  &  $  2454381.80583$  &  $  0.9833$ \\
  $  1$  &  $  2454381.80633$  &  $  0.9857$ \\
  $  1$  &  $  2454381.80683$  &  $  0.9895$ \\
  $  1$  &  $  2454381.80734$  &  $  0.9826$ \\
  $  1$  &  $  2454381.80784$  &  $  0.9862$ \\
  $  1$  &  $  2454381.80834$  &  $  0.9839$ \\
  $  1$  &  $  2454381.80885$  &  $  0.9860$ \\
  $  1$  &  $  2454381.80935$  &  $  0.9850$ \\
  $  1$  &  $  2454381.80985$  &  $  0.9841$ \\
  $  1$  &  $  2454381.81036$  &  $  0.9839$ \\
  $  1$  &  $  2454381.81086$  &  $  0.9848$ \\
  $  1$  &  $  2454381.81136$  &  $  0.9856$ \\
  $  1$  &  $  2454381.81196$  &  $  0.9873$ \\
  $  1$  &  $  2454381.81247$  &  $  0.9819$ \\
  $  1$  &  $  2454381.81298$  &  $  0.9862$ \\
  $  1$  &  $  2454381.81348$  &  $  0.9858$ \\
  $  1$  &  $  2454381.81398$  &  $  0.9865$ \\
  $  1$  &  $  2454381.81448$  &  $  0.9875$ \\
  $  1$  &  $  2454381.81499$  &  $  0.9868$ \\
  $  1$  &  $  2454381.81549$  &  $  0.9851$ \\
  $  1$  &  $  2454381.81600$  &  $  0.9875$ \\
  $  1$  &  $  2454381.81650$  &  $  0.9894$ \\
  $  1$  &  $  2454381.81700$  &  $  0.9840$ \\
  $  1$  &  $  2454381.81751$  &  $  0.9845$ \\
  $  1$  &  $  2454381.81801$  &  $  0.9854$ \\
  $  1$  &  $  2454381.81851$  &  $  0.9862$ \\
  $  1$  &  $  2454381.81902$  &  $  0.9894$ \\
  $  1$  &  $  2454381.81952$  &  $  0.9850$ \\
  $  1$  &  $  2454381.82002$  &  $  0.9854$ \\
  $  1$  &  $  2454381.82053$  &  $  0.9858$ \\
  $  1$  &  $  2454381.82103$  &  $  0.9896$ \\
  $  1$  &  $  2454381.82153$  &  $  0.9852$ \\
  $  1$  &  $  2454381.82214$  &  $  0.9878$ \\
  $  1$  &  $  2454381.82264$  &  $  0.9831$ \\
  $  1$  &  $  2454381.82314$  &  $  0.9868$ \\
  $  1$  &  $  2454381.82365$  &  $  0.9845$ \\
  $  1$  &  $  2454381.82415$  &  $  0.9888$ \\
  $  1$  &  $  2454381.82466$  &  $  0.9898$ \\
  $  1$  &  $  2454381.82516$  &  $  0.9869$ \\
  $  1$  &  $  2454381.82566$  &  $  0.9857$ \\
  $  1$  &  $  2454381.82616$  &  $  0.9862$ \\
  $  1$  &  $  2454381.82667$  &  $  0.9835$ \\
  $  1$  &  $  2454381.82717$  &  $  0.9887$ \\
  $  1$  &  $  2454381.82767$  &  $  0.9884$ \\
  $  1$  &  $  2454381.82818$  &  $  0.9860$ \\
  $  1$  &  $  2454381.82868$  &  $  0.9833$ \\
  $  1$  &  $  2454381.82919$  &  $  0.9877$ \\
  $  1$  &  $  2454381.82969$  &  $  0.9866$ \\
  $  1$  &  $  2454381.83019$  &  $  0.9870$ \\
  $  1$  &  $  2454381.83070$  &  $  0.9852$ \\
  $  1$  &  $  2454381.83120$  &  $  0.9848$ \\
  $  1$  &  $  2454381.83170$  &  $  0.9884$ \\
  $  1$  &  $  2454381.83233$  &  $  0.9867$ \\
  $  1$  &  $  2454381.83284$  &  $  0.9859$ \\
  $  1$  &  $  2454381.83334$  &  $  0.9860$ \\
  $  1$  &  $  2454381.83384$  &  $  0.9898$ \\
  $  1$  &  $  2454381.83435$  &  $  0.9885$ \\
  $  1$  &  $  2454381.83485$  &  $  0.9855$ \\
  $  1$  &  $  2454381.83536$  &  $  0.9881$ \\
  $  1$  &  $  2454381.83586$  &  $  0.9895$ \\
  $  1$  &  $  2454381.83636$  &  $  0.9892$ \\
  $  1$  &  $  2454381.83687$  &  $  0.9877$ \\
  $  1$  &  $  2454381.83737$  &  $  0.9873$ \\
  $  1$  &  $  2454381.83787$  &  $  0.9875$ \\
  $  1$  &  $  2454381.83838$  &  $  0.9867$ \\
  $  1$  &  $  2454381.83888$  &  $  0.9896$ \\
  $  1$  &  $  2454381.83938$  &  $  0.9865$ \\
  $  1$  &  $  2454381.83989$  &  $  0.9913$ \\
  $  1$  &  $  2454381.84039$  &  $  0.9885$ \\
  $  1$  &  $  2454381.84089$  &  $  0.9863$ \\
  $  1$  &  $  2454381.84140$  &  $  0.9888$ \\
  $  1$  &  $  2454381.84190$  &  $  0.9868$ \\
  $  1$  &  $  2454381.84254$  &  $  0.9913$ \\
  $  1$  &  $  2454381.84304$  &  $  0.9883$ \\
  $  1$  &  $  2454381.84355$  &  $  0.9865$ \\
  $  1$  &  $  2454381.84405$  &  $  0.9851$ \\
  $  1$  &  $  2454381.84455$  &  $  0.9919$ \\
  $  1$  &  $  2454381.84506$  &  $  0.9869$ \\
  $  1$  &  $  2454381.84556$  &  $  0.9878$ \\
  $  1$  &  $  2454381.84606$  &  $  0.9900$ \\
  $  1$  &  $  2454381.84657$  &  $  0.9883$ \\
  $  1$  &  $  2454381.84707$  &  $  0.9888$ \\
  $  1$  &  $  2454381.84757$  &  $  0.9891$ \\
  $  1$  &  $  2454381.84808$  &  $  0.9905$ \\
  $  1$  &  $  2454381.84858$  &  $  0.9901$ \\
  $  1$  &  $  2454381.84908$  &  $  0.9888$ \\
  $  1$  &  $  2454381.84959$  &  $  0.9892$ \\
  $  1$  &  $  2454381.85009$  &  $  0.9917$ \\
  $  1$  &  $  2454381.85060$  &  $  0.9914$ \\
  $  1$  &  $  2454381.85110$  &  $  0.9921$ \\
  $  1$  &  $  2454381.85160$  &  $  0.9947$ \\
  $  1$  &  $  2454381.85211$  &  $  0.9913$ \\
  $  1$  &  $  2454381.85266$  &  $  0.9938$ \\
  $  1$  &  $  2454381.85317$  &  $  0.9978$ \\
  $  1$  &  $  2454381.85367$  &  $  0.9888$ \\
  $  1$  &  $  2454381.85417$  &  $  0.9902$ \\
  $  1$  &  $  2454381.85468$  &  $  0.9958$ \\
  $  1$  &  $  2454381.85518$  &  $  0.9942$ \\
  $  1$  &  $  2454381.85568$  &  $  0.9978$ \\
  $  1$  &  $  2454381.85619$  &  $  0.9972$ \\
  $  1$  &  $  2454381.85669$  &  $  0.9959$ \\
  $  1$  &  $  2454381.85720$  &  $  0.9973$ \\
  $  1$  &  $  2454381.85770$  &  $  0.9945$ \\
  $  1$  &  $  2454381.85820$  &  $  0.9981$ \\
  $  1$  &  $  2454381.85871$  &  $  0.9987$ \\
  $  1$  &  $  2454381.85921$  &  $  0.9962$ \\
  $  1$  &  $  2454381.85971$  &  $  0.9962$ \\
  $  1$  &  $  2454381.86022$  &  $  0.9967$ \\
  $  1$  &  $  2454381.86072$  &  $  0.9962$ \\
  $  1$  &  $  2454381.86124$  &  $  1.0018$ \\
  $  1$  &  $  2454381.86174$  &  $  1.0003$ \\
  $  1$  &  $  2454381.86225$  &  $  0.9994$ \\
  $  1$  &  $  2454381.86287$  &  $  0.9958$ \\
  $  1$  &  $  2454381.86337$  &  $  0.9989$ \\
  $  1$  &  $  2454381.86387$  &  $  0.9988$ \\
  $  1$  &  $  2454381.86438$  &  $  1.0005$ \\
  $  1$  &  $  2454381.86488$  &  $  0.9989$ \\
  $  1$  &  $  2454381.86538$  &  $  0.9985$ \\
  $  1$  &  $  2454381.86589$  &  $  1.0012$ \\
  $  1$  &  $  2454381.86639$  &  $  1.0000$ \\
  $  1$  &  $  2454381.86689$  &  $  1.0002$ \\
  $  1$  &  $  2454381.86740$  &  $  0.9959$ \\
  $  1$  &  $  2454381.86790$  &  $  1.0056$ \\
  $  1$  &  $  2454381.86840$  &  $  1.0006$ \\
  $  1$  &  $  2454381.86891$  &  $  0.9972$ \\
  $  1$  &  $  2454381.86941$  &  $  1.0016$ \\
  $  1$  &  $  2454381.86991$  &  $  1.0046$ \\
  $  1$  &  $  2454381.87042$  &  $  1.0001$ \\
  $  1$  &  $  2454381.87092$  &  $  1.0005$ \\
  $  1$  &  $  2454381.87143$  &  $  1.0018$ \\
  $  1$  &  $  2454381.87193$  &  $  0.9994$ \\
  $  1$  &  $  2454381.87243$  &  $  1.0029$ \\
  $  1$  &  $  2454381.87305$  &  $  0.9995$ \\
  $  1$  &  $  2454381.87355$  &  $  1.0025$ \\
  $  1$  &  $  2454381.87406$  &  $  1.0007$ \\
  $  1$  &  $  2454381.87456$  &  $  1.0019$ \\
  $  1$  &  $  2454381.87506$  &  $  0.9990$ \\
  $  1$  &  $  2454381.87557$  &  $  1.0008$ \\
  $  1$  &  $  2454381.87607$  &  $  1.0030$ \\
  $  1$  &  $  2454381.87658$  &  $  1.0016$ \\
  $  1$  &  $  2454381.87708$  &  $  1.0020$ \\
  $  1$  &  $  2454381.87758$  &  $  1.0014$ \\
  $  1$  &  $  2454381.87826$  &  $  1.0023$ \\
  $  1$  &  $  2454381.87877$  &  $  0.9998$ \\
  $  1$  &  $  2454381.87928$  &  $  0.9980$ \\
  $  1$  &  $  2454381.87978$  &  $  1.0012$ \\
  $  1$  &  $  2454381.88028$  &  $  0.9990$ \\
  $  1$  &  $  2454381.88079$  &  $  1.0044$ \\
  $  1$  &  $  2454381.88129$  &  $  1.0024$ \\
  $  1$  &  $  2454381.88179$  &  $  0.9996$ \\
  $  1$  &  $  2454381.88230$  &  $  1.0015$ \\
  $  1$  &  $  2454381.88280$  &  $  0.9988$ \\
  $  2$  &  $  2454363.83094$  &  $  1.0006$ \\
  $  2$  &  $  2454363.83151$  &  $  1.0006$ \\
  $  2$  &  $  2454363.83260$  &  $  0.9973$ \\
  $  2$  &  $  2454363.83316$  &  $  1.0004$ \\
  $  2$  &  $  2454363.83373$  &  $  0.9984$ \\
  $  2$  &  $  2454363.83493$  &  $  1.0007$ \\
  $  2$  &  $  2454363.83551$  &  $  1.0024$ \\
  $  2$  &  $  2454363.83681$  &  $  1.0006$ \\
  $  2$  &  $  2454363.83734$  &  $  0.9978$ \\
  $  2$  &  $  2454363.83795$  &  $  1.0004$ \\
  $  2$  &  $  2454363.83847$  &  $  1.0019$ \\
  $  2$  &  $  2454363.83902$  &  $  0.9976$ \\
  $  2$  &  $  2454363.84014$  &  $  1.0011$ \\
  $  2$  &  $  2454363.84124$  &  $  1.0052$ \\
  $  2$  &  $  2454363.84251$  &  $  1.0024$ \\
  $  2$  &  $  2454363.84306$  &  $  1.0015$ \\
  $  2$  &  $  2454363.84358$  &  $  1.0004$ \\
  $  2$  &  $  2454363.84416$  &  $  1.0009$ \\
  $  2$  &  $  2454363.84474$  &  $  0.9994$ \\
  $  2$  &  $  2454363.84529$  &  $  0.9984$ \\
  $  2$  &  $  2454363.84582$  &  $  0.9983$ \\
  $  2$  &  $  2454363.84637$  &  $  1.0015$ \\
  $  2$  &  $  2454363.84694$  &  $  0.9978$ \\
  $  2$  &  $  2454363.84827$  &  $  0.9996$ \\
  $  2$  &  $  2454363.84880$  &  $  1.0014$ \\
  $  2$  &  $  2454363.84932$  &  $  1.0004$ \\
  $  2$  &  $  2454363.85044$  &  $  0.9994$ \\
  $  2$  &  $  2454363.85098$  &  $  0.9974$ \\
  $  2$  &  $  2454363.85151$  &  $  1.0010$ \\
  $  2$  &  $  2454363.85206$  &  $  1.0006$ \\
  $  2$  &  $  2454363.85264$  &  $  0.9977$ \\
  $  2$  &  $  2454363.85394$  &  $  0.9996$ \\
  $  2$  &  $  2454363.85447$  &  $  0.9977$ \\
  $  2$  &  $  2454363.85501$  &  $  0.9976$ \\
  $  2$  &  $  2454363.85559$  &  $  1.0018$ \\
  $  2$  &  $  2454363.85611$  &  $  1.0021$ \\
  $  2$  &  $  2454363.85667$  &  $  1.0002$ \\
  $  2$  &  $  2454363.85723$  &  $  1.0001$ \\
  $  2$  &  $  2454363.85778$  &  $  1.0033$ \\
  $  2$  &  $  2454363.85834$  &  $  0.9996$ \\
  $  2$  &  $  2454363.85973$  &  $  0.9986$ \\
  $  2$  &  $  2454363.86035$  &  $  1.0005$ \\
  $  2$  &  $  2454363.86099$  &  $  0.9994$ \\
  $  2$  &  $  2454363.86159$  &  $  0.9990$ \\
  $  2$  &  $  2454363.86212$  &  $  1.0012$ \\
  $  2$  &  $  2454363.86275$  &  $  1.0020$ \\
  $  2$  &  $  2454363.86654$  &  $  1.0014$ \\
  $  2$  &  $  2454363.86716$  &  $  0.9995$ \\
  $  2$  &  $  2454363.86923$  &  $  0.9999$ \\
  $  2$  &  $  2454363.86978$  &  $  0.9984$ \\
  $  2$  &  $  2454363.87037$  &  $  1.0010$ \\
  $  2$  &  $  2454363.87098$  &  $  1.0019$ \\
  $  2$  &  $  2454363.87159$  &  $  0.9987$ \\
  $  2$  &  $  2454363.87218$  &  $  0.9995$ \\
  $  2$  &  $  2454363.87356$  &  $  0.9995$ \\
  $  2$  &  $  2454363.87424$  &  $  1.0023$ \\
  $  2$  &  $  2454363.87488$  &  $  1.0012$ \\
  $  2$  &  $  2454363.87548$  &  $  1.0017$ \\
  $  2$  &  $  2454363.87604$  &  $  1.0002$ \\
  $  2$  &  $  2454363.87717$  &  $  1.0009$ \\
  $  2$  &  $  2454363.87777$  &  $  0.9996$ \\
  $  2$  &  $  2454363.87836$  &  $  0.9995$ \\
  $  2$  &  $  2454363.88037$  &  $  1.0023$ \\
  $  2$  &  $  2454363.88104$  &  $  1.0012$ \\
  $  2$  &  $  2454363.88168$  &  $  0.9999$ \\
  $  2$  &  $  2454363.88227$  &  $  1.0011$ \\
  $  2$  &  $  2454363.88283$  &  $  1.0028$ \\
  $  2$  &  $  2454363.88336$  &  $  0.9991$ \\
  $  2$  &  $  2454363.88398$  &  $  1.0005$ \\
  $  2$  &  $  2454363.88726$  &  $  1.0011$ \\
  $  2$  &  $  2454363.88784$  &  $  0.9998$ \\
  $  2$  &  $  2454363.88842$  &  $  1.0011$ \\
  $  2$  &  $  2454363.88897$  &  $  1.0000$ \\
  $  2$  &  $  2454363.88954$  &  $  1.0009$ \\
  $  2$  &  $  2454363.89014$  &  $  0.9986$ \\
  $  2$  &  $  2454363.89071$  &  $  0.9985$ \\
  $  2$  &  $  2454363.89209$  &  $  0.9976$ \\
  $  2$  &  $  2454363.89273$  &  $  0.9985$ \\
  $  2$  &  $  2454363.89339$  &  $  0.9993$ \\
  $  2$  &  $  2454363.89403$  &  $  0.9980$ \\
  $  2$  &  $  2454363.89467$  &  $  0.9956$ \\
  $  2$  &  $  2454363.89591$  &  $  0.9972$ \\
  $  2$  &  $  2454363.89655$  &  $  0.9977$ \\
  $  2$  &  $  2454363.89714$  &  $  0.9948$ \\
  $  2$  &  $  2454363.90086$  &  $  0.9939$ \\
  $  2$  &  $  2454363.90145$  &  $  0.9956$ \\
  $  2$  &  $  2454363.90202$  &  $  0.9952$ \\
  $  2$  &  $  2454363.90258$  &  $  0.9937$ \\
  $  2$  &  $  2454363.90316$  &  $  0.9954$ \\
  $  2$  &  $  2454363.90375$  &  $  0.9898$ \\
  $  2$  &  $  2454363.90438$  &  $  0.9940$ \\
  $  2$  &  $  2454363.90496$  &  $  0.9939$ \\
  $  2$  &  $  2454363.90711$  &  $  0.9911$ \\
  $  2$  &  $  2454363.90776$  &  $  0.9921$ \\
  $  2$  &  $  2454363.90841$  &  $  0.9919$ \\
  $  2$  &  $  2454363.90904$  &  $  0.9897$ \\
  $  2$  &  $  2454363.90963$  &  $  0.9900$ \\
  $  2$  &  $  2454363.91023$  &  $  0.9872$ \\
  $  2$  &  $  2454363.91083$  &  $  0.9880$ \\
  $  2$  &  $  2454363.91144$  &  $  0.9903$ \\
  $  2$  &  $  2454363.91198$  &  $  0.9875$ \\
  $  2$  &  $  2454363.91364$  &  $  0.9884$ \\
  $  2$  &  $  2454363.91427$  &  $  0.9893$ \\
  $  2$  &  $  2454363.91495$  &  $  0.9891$ \\
  $  2$  &  $  2454363.91559$  &  $  0.9869$ \\
  $  2$  &  $  2454363.91621$  &  $  0.9873$ \\
  $  2$  &  $  2454363.91683$  &  $  0.9908$ \\
  $  2$  &  $  2454363.91746$  &  $  0.9871$ \\
  $  2$  &  $  2454363.91801$  &  $  0.9866$ \\
  $  2$  &  $  2454363.91858$  &  $  0.9847$ \\
  $  2$  &  $  2454363.92011$  &  $  0.9865$ \\
  $  2$  &  $  2454363.92078$  &  $  0.9884$ \\
  $  2$  &  $  2454363.92143$  &  $  0.9873$ \\
  $  2$  &  $  2454363.92209$  &  $  0.9851$ \\
  $  2$  &  $  2454363.92271$  &  $  0.9863$ \\
  $  2$  &  $  2454363.92331$  &  $  0.9889$ \\
  $  2$  &  $  2454363.92394$  &  $  0.9852$ \\
  $  2$  &  $  2454363.92454$  &  $  0.9884$ \\
  $  2$  &  $  2454363.92513$  &  $  0.9838$ \\
  $  2$  &  $  2454363.92657$  &  $  0.9883$ \\
  $  2$  &  $  2454363.92724$  &  $  0.9883$ \\
  $  2$  &  $  2454363.92789$  &  $  0.9854$ \\
  $  2$  &  $  2454363.92855$  &  $  0.9842$ \\
  $  2$  &  $  2454363.92917$  &  $  0.9854$ \\
  $  2$  &  $  2454363.92980$  &  $  0.9871$ \\
  $  2$  &  $  2454363.93039$  &  $  0.9852$ \\
  $  2$  &  $  2454363.93103$  &  $  0.9875$ \\
  $  2$  &  $  2454363.93166$  &  $  0.9847$ \\
  $  2$  &  $  2454363.93314$  &  $  0.9856$ \\
  $  2$  &  $  2454363.93440$  &  $  0.9863$ \\
  $  2$  &  $  2454363.93506$  &  $  0.9869$ \\
  $  2$  &  $  2454363.93571$  &  $  0.9845$ \\
  $  2$  &  $  2454363.93636$  &  $  0.9880$ \\
  $  2$  &  $  2454363.93695$  &  $  0.9879$ \\
  $  2$  &  $  2454363.93755$  &  $  0.9838$ \\
  $  2$  &  $  2454363.93814$  &  $  0.9865$ \\
  $  2$  &  $  2454363.93960$  &  $  0.9892$ \\
  $  2$  &  $  2454363.94025$  &  $  0.9847$ \\
  $  2$  &  $  2454363.94092$  &  $  0.9854$ \\
  $  2$  &  $  2454363.94158$  &  $  0.9850$ \\
  $  2$  &  $  2454363.94223$  &  $  0.9844$ \\
  $  2$  &  $  2454363.94284$  &  $  0.9834$ \\
  $  2$  &  $  2454363.94344$  &  $  0.9851$ \\
  $  2$  &  $  2454363.94405$  &  $  0.9893$ \\
  $  2$  &  $  2454363.94466$  &  $  0.9865$ \\
  $  2$  &  $  2454363.94680$  &  $  0.9828$ \\
  $  2$  &  $  2454363.94743$  &  $  0.9846$ \\
  $  2$  &  $  2454363.94812$  &  $  0.9836$ \\
  $  2$  &  $  2454363.94877$  &  $  0.9850$ \\
  $  2$  &  $  2454363.94932$  &  $  0.9880$ \\
  $  2$  &  $  2454363.94995$  &  $  0.9870$ \\
  $  2$  &  $  2454363.95056$  &  $  0.9869$ \\
  $  2$  &  $  2454363.95115$  &  $  0.9856$ \\
  $  2$  &  $  2454363.95179$  &  $  0.9873$ \\
  $  2$  &  $  2454363.95338$  &  $  0.9873$ \\
  $  2$  &  $  2454363.95403$  &  $  0.9855$ \\
  $  2$  &  $  2454363.95471$  &  $  0.9854$ \\
  $  2$  &  $  2454363.95537$  &  $  0.9850$ \\
  $  2$  &  $  2454363.95602$  &  $  0.9835$ \\
  $  2$  &  $  2454363.95662$  &  $  0.9843$ \\
  $  2$  &  $  2454363.95725$  &  $  0.9860$ \\
  $  2$  &  $  2454363.95784$  &  $  0.9874$ \\
  $  2$  &  $  2454363.95843$  &  $  0.9855$ \\
  $  2$  &  $  2454363.96000$  &  $  0.9828$ \\
  $  2$  &  $  2454363.96064$  &  $  0.9873$ \\
  $  2$  &  $  2454363.96131$  &  $  0.9844$ \\
  $  2$  &  $  2454363.96198$  &  $  0.9877$ \\
  $  2$  &  $  2454363.96261$  &  $  0.9871$ \\
  $  2$  &  $  2454363.96319$  &  $  0.9861$ \\
  $  2$  &  $  2454363.96380$  &  $  0.9869$ \\
  $  2$  &  $  2454363.96439$  &  $  0.9874$ \\
  $  2$  &  $  2454363.96499$  &  $  0.9855$ \\
  $  2$  &  $  2454363.96651$  &  $  0.9855$ \\
  $  2$  &  $  2454363.96716$  &  $  0.9891$ \\
  $  2$  &  $  2454363.96786$  &  $  0.9889$ \\
  $  2$  &  $  2454363.96853$  &  $  0.9877$ \\
  $  2$  &  $  2454363.96917$  &  $  0.9853$ \\
  $  2$  &  $  2454363.96978$  &  $  0.9879$ \\
  $  2$  &  $  2454363.97037$  &  $  0.9869$ \\
  $  2$  &  $  2454363.97096$  &  $  0.9901$ \\
  $  2$  &  $  2454363.97157$  &  $  0.9891$ \\
  $  2$  &  $  2454363.97315$  &  $  0.9900$ \\
  $  2$  &  $  2454363.97386$  &  $  0.9891$ \\
  $  2$  &  $  2454363.97451$  &  $  0.9889$ \\
  $  2$  &  $  2454363.97515$  &  $  0.9895$ \\
  $  2$  &  $  2454363.97579$  &  $  0.9880$ \\
  $  2$  &  $  2454363.97643$  &  $  0.9887$ \\
  $  2$  &  $  2454363.97703$  &  $  0.9905$ \\
  $  2$  &  $  2454363.97764$  &  $  0.9901$ \\
  $  2$  &  $  2454363.97826$  &  $  0.9882$ \\
  $  2$  &  $  2454363.97974$  &  $  0.9882$ \\
  $  2$  &  $  2454363.98048$  &  $  0.9863$ \\
  $  2$  &  $  2454363.98115$  &  $  0.9889$ \\
  $  2$  &  $  2454363.98180$  &  $  0.9894$ \\
  $  2$  &  $  2454363.98245$  &  $  0.9870$ \\
  $  2$  &  $  2454363.98304$  &  $  0.9915$ \\
  $  2$  &  $  2454363.98365$  &  $  0.9868$ \\
  $  2$  &  $  2454363.98430$  &  $  0.9919$ \\
  $  2$  &  $  2454363.98485$  &  $  0.9909$ \\
  $  2$  &  $  2454363.98704$  &  $  0.9909$ \\
  $  2$  &  $  2454363.98772$  &  $  0.9927$ \\
  $  2$  &  $  2454363.98844$  &  $  0.9934$ \\
  $  2$  &  $  2454363.98911$  &  $  0.9931$ \\
  $  2$  &  $  2454363.98969$  &  $  0.9934$ \\
  $  2$  &  $  2454363.99035$  &  $  0.9942$ \\
  $  2$  &  $  2454363.99252$  &  $  0.9950$ \\
  $  2$  &  $  2454363.99313$  &  $  0.9955$ \\
  $  2$  &  $  2454363.99380$  &  $  0.9954$ \\
  $  2$  &  $  2454363.99542$  &  $  0.9963$ \\
  $  2$  &  $  2454363.99612$  &  $  0.9982$ \\
  $  2$  &  $  2454363.99679$  &  $  0.9989$ \\
  $  2$  &  $  2454363.99750$  &  $  0.9985$ \\
  $  2$  &  $  2454363.99821$  &  $  1.0007$ \\
  $  2$  &  $  2454363.99893$  &  $  0.9997$ \\
  $  2$  &  $  2454363.99961$  &  $  0.9987$ \\
  $  2$  &  $  2454364.00029$  &  $  0.9973$ \\
  $  2$  &  $  2454364.00091$  &  $  0.9981$ \\
  $  2$  &  $  2454364.00252$  &  $  1.0009$ \\
  $  2$  &  $  2454364.00320$  &  $  0.9981$ \\
  $  2$  &  $  2454364.00395$  &  $  1.0007$ \\
  $  2$  &  $  2454364.00465$  &  $  1.0013$ \\
  $  2$  &  $  2454364.00535$  &  $  1.0016$ \\
  $  2$  &  $  2454364.00601$  &  $  0.9996$ \\
  $  2$  &  $  2454364.00671$  &  $  0.9995$ \\
  $  2$  &  $  2454364.00734$  &  $  0.9991$ \\
  $  2$  &  $  2454364.00791$  &  $  1.0000$ \\
  $  2$  &  $  2454364.00959$  &  $  1.0018$ \\
  $  2$  &  $  2454364.01028$  &  $  0.9990$ \\
  $  2$  &  $  2454364.01098$  &  $  0.9998$ \\
  $  2$  &  $  2454364.01171$  &  $  0.9985$ \\
  $  2$  &  $  2454364.01241$  &  $  1.0034$ \\
  $  2$  &  $  2454364.01311$  &  $  1.0051$ \\
  $  2$  &  $  2454364.01372$  &  $  1.0004$ \\
  $  2$  &  $  2454364.01436$  &  $  1.0000$ \\
  $  2$  &  $  2454364.01502$  &  $  1.0036$ \\
  $  2$  &  $  2454364.01657$  &  $  0.9990$ \\
  $  2$  &  $  2454364.01724$  &  $  1.0008$ \\
  $  2$  &  $  2454364.01792$  &  $  1.0034$ \\
  $  2$  &  $  2454364.01865$  &  $  1.0012$ \\
  $  2$  &  $  2454364.01932$  &  $  0.9997$ \\
  $  2$  &  $  2454364.02004$  &  $  0.9996$ \\
  $  2$  &  $  2454364.02069$  &  $  0.9995$ \\
  $  2$  &  $  2454364.02136$  &  $  0.9991$ \\
  $  2$  &  $  2454364.02201$  &  $  0.9999$ \\
  $  2$  &  $  2454364.02378$  &  $  0.9999$ \\
  $  2$  &  $  2454364.02459$  &  $  1.0027$ \\
  $  2$  &  $  2454364.02528$  &  $  0.9988$ \\
  $  2$  &  $  2454364.02594$  &  $  1.0003$ \\
  $  2$  &  $  2454364.02666$  &  $  0.9997$ \\
  $  2$  &  $  2454364.02727$  &  $  0.9986$ \\
  $  2$  &  $  2454364.02790$  &  $  1.0013$ \\
  $  2$  &  $  2454364.02853$  &  $  1.0000$ \\
  $  2$  &  $  2454364.02922$  &  $  0.9980$ \\

